The SAGEX Review on Scattering Amplitudes

This is an introduction to, and invitation to read, a series of review articles on scattering amplitudes in gauge theory, gravity, and superstring theory. Our aim is to provide an overview of the field, from basic aspects to a selection of current (2022) research and developments.

==> SAGEX review - chapter 0/tikz.tex <==
\usetikzlibrary{calc,arrows, decorations.markings, shapes.misc, decorations.pathmorphing}

\def\arrowstyle{latex}       % arrow style for each internal line: (latex, stealth, >)
\def\boxsize{0.7}
\def\blobsize{0.55cm}
\def\bwblobsize{0.35cm}

\tikzset{
  ->-/.style={
    decoration={
      markings,
      mark=at position #1 with {\arrow{latex}}},
    postaction={decorate}
  },
  ->-/.default=0.5
}

\tikzset{
    wavy/.style={decorate, decoration={snake}, draw=red},
}

\tikzset{VO/.style={cross out, draw, 
         minimum size=5pt, 
         inner sep=0pt, outer sep=0pt}}

\tikzset{VOline/.style={decorate, decoration={snake}},
}

\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}

%%%%% ON-SHELL %%%%%

\newcommand{\blackdot}{\node[circle, fill=black, draw, inner sep=0pt, minimum size=\bwblobsize]}
\newcommand{\whitedot}{\node[circle, fill=white, draw, inner sep=0pt, minimum size=\bwblobsize]}
\newcommand{\greyblob}{\node[circle, fill=black!20, draw, inner sep=2pt, minimum size=\blobsize]}


%%%%% BOXES %%%%%%

\newcommand{\drawULblack}{\blackdot (UL) at (-\boxsize,  \boxsize) {};}
\newcommand{\drawURblack}{\blackdot (UR) at ( \boxsize,  \boxsize) {};}
\newcommand{\drawLRblack}{\blackdot (LR) at ( \boxsize, -\boxsize) {};}
\newcommand{\drawLLblack}{\blackdot (LL) at (-\boxsize, -\boxsize) {};}

\newcommand{\drawULwhite}{\whitedot (UL) at (-\boxsize,  \boxsize) {};}
\newcommand{\drawURwhite}{\whitedot (UR) at ( \boxsize,  \boxsize) {};}
\newcommand{\drawLRwhite}{\whitedot (LR) at ( \boxsize, -\boxsize) {};}
\newcommand{\drawLLwhite}{\whitedot (LL) at (-\boxsize, -\boxsize) {};}

\newcommand{\drawUL}[1]{\greyblob (UL) at (-\boxsize,  \boxsize) {#1};}
\newcommand{\drawUR}[1]{\greyblob (UR) at ( \boxsize,  \boxsize) {#1};}
\newcommand{\drawLR}[1]{\greyblob (LR) at ( \boxsize, -\boxsize) {#1};}
\newcommand{\drawLL}[1]{\greyblob (LL) at (-\boxsize, -\boxsize) {#1};}

\newcommand{\drawULempty}{\coordinate (UL) at (-\boxsize,  \boxsize);}
\newcommand{\drawURempty}{\coordinate (UR) at ( \boxsize,  \boxsize);}
\newcommand{\drawLRempty}{\coordinate (LR) at ( \boxsize, -\boxsize);}
\newcommand{\drawLLempty}{\coordinate (LL) at (-\boxsize, -\boxsize);}

\newcommand{\drawboxinternallines}{
  \draw (UL) -- (UR) -- (LR) -- (LL) -- (UL);
}

\newcommand{\drawinternalmomenta}{
  \draw[->] (+0.3, -1.1) -- (-0.3, -1.1) node[anchor=north west] {$\lone$};
  \draw[->] (-1.1, -0.3) -- (-1.1, +0.3) node[anchor=north east] {$\ltwo$};
  \draw[->] (-0.3, +1.1) -- (+0.3, +1.1) node[anchor=south east] {$\lthree$};
  \draw[->] (+1.1, +0.3) -- (+1.1, -0.3) node[anchor=south west] {$\lfour$};
}

\newcommand{\drawregionvariables}[5]{
  \draw ( 0.0, -1.4) node {#1};
  \draw (-1.4,  0.0) node {#2};
  \draw ( 0.0,  1.4) node {#3};
  \draw ( 1.4,  0.0) node {#4};
  \draw ( 0.0,  0.0) node {#5};
}

%%%%% BCFW %%%%%%

\newcommand{\drawLblack}{\node[circle, fill=black, draw, minimum size=0.3cm] (L) at (-0.9,  0.0) {};}
\newcommand{\drawRblack}{\node[circle, fill=black, draw, minimum size=0.3cm] (R) at ( 0.9,  0.0) {};}

\newcommand{\drawLwhite}{\node[circle, fill=white, draw, minimum size=0.3cm] (L) at (-0.9,  0.0) {};}
\newcommand{\drawRwhite}{\node[circle, fill=white, draw, minimum size=0.3cm] (R) at ( 0.9,  0.0) {};}

\newcommand{\drawL}[1]{\node[circle, fill=black!20, draw, minimum size=0.5cm, inner sep=2pt] (L) at (-0.9,  0.0) {#1};}
\newcommand{\drawR}[1]{\node[circle, fill=black!20, draw, minimum size=0.5cm, inner sep=2pt] (R) at ( 0.9,  0.0) {#1};}

\newcommand{\drawBCFWinternalline}{
  \draw (L) -- ++( 0.8,  0.0);
  \draw (R) -- ++(-0.8,  0.0);
}

%%%%% MHV %%%%%%

\newcommand{\drawblobs}{
\node[circle, fill=black!20, draw, minimum size=0.6cm] (blobL) at (-1, 0) {};
\node[circle, fill=black!20, draw, minimum size=0.6cm] (blobR) at (+1, 0) {};
}

\newcommand{\drawupperlower}{
\draw (blobL) to[out=60, in=120] (blobR);
\draw (blobL) to[out=-60, in=-120] (blobR);
}

\newcommand{\drawuppercross}{
\draw (blobL) to[out=60, in=120] node[cross out, draw=red]{} (blobR);
}

\newcommand{\drawlowercross}{
\draw (blobL) to[out=-60, in=-120] node[cross out, draw=red]{} (blobR);
}

\newcommand{\drawuppercut}{
\draw (blobL) to[out=60, in=120] node[circle, fill=white, draw=white]{} (blobR);
\draw[red, dashed] (0, 0.4) -- (0, 1.0);
}

\newcommand{\drawlowercut}{
\draw (blobL) to[out=-60, in=-120] node[circle, fill=white, draw=white]{} (blobR);
\draw[red, dashed] (0,-0.4) -- (0,-1.0);
}


==> tikz.tex <==
\usetikzlibrary{calc,arrows, decorations.markings, shapes.misc, decorations.pathmorphing}

\def\arrowstyle{latex}       % arrow style for each internal line: (latex, stealth, >)
\def\boxsize{0.7}
\def\blobsize{0.55cm}
\def\bwblobsize{0.35cm}

\tikzset{
  ->-/.style={
    decoration={
      markings,
      mark=at position #1 with {\arrow{latex}}},
    postaction={decorate}
  },
  ->-/.default=0.5
}

\tikzset{
    wavy/.style={decorate, decoration={snake}, draw=red},
}

\tikzset{VO/.style={cross out, draw, 
         minimum size=5pt, 
         inner sep=0pt, outer sep=0pt}}

\tikzset{VOline/.style={decorate, decoration={snake}},
}

\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}

%%%%% ON-SHELL %%%%%

\newcommand{\blackdot}{\node[circle, fill=black, draw, inner sep=0pt, minimum size=\bwblobsize]}
\newcommand{\whitedot}{\node[circle, fill=white, draw, inner sep=0pt, minimum size=\bwblobsize]}
\newcommand{\greyblob}{\node[circle, fill=black!20, draw, inner sep=2pt, minimum size=\blobsize]}


%%%%% BOXES %%%%%%

\newcommand{\drawULblack}{\blackdot (UL) at (-\boxsize,  \boxsize) {};}
\newcommand{\drawURblack}{\blackdot (UR) at ( \boxsize,  \boxsize) {};}
\newcommand{\drawLRblack}{\blackdot (LR) at ( \boxsize, -\boxsize) {};}
\newcommand{\drawLLblack}{\blackdot (LL) at (-\boxsize, -\boxsize) {};}

\newcommand{\drawULwhite}{\whitedot (UL) at (-\boxsize,  \boxsize) {};}
\newcommand{\drawURwhite}{\whitedot (UR) at ( \boxsize,  \boxsize) {};}
\newcommand{\drawLRwhite}{\whitedot (LR) at ( \boxsize, -\boxsize) {};}
\newcommand{\drawLLwhite}{\whitedot (LL) at (-\boxsize, -\boxsize) {};}

\newcommand{\drawUL}[1]{\greyblob (UL) at (-\boxsize,  \boxsize) {#1};}
\newcommand{\drawUR}[1]{\greyblob (UR) at ( \boxsize,  \boxsize) {#1};}
\newcommand{\drawLR}[1]{\greyblob (LR) at ( \boxsize, -\boxsize) {#1};}
\newcommand{\drawLL}[1]{\greyblob (LL) at (-\boxsize, -\boxsize) {#1};}

\newcommand{\drawULempty}{\coordinate (UL) at (-\boxsize,  \boxsize);}
\newcommand{\drawURempty}{\coordinate (UR) at ( \boxsize,  \boxsize);}
\newcommand{\drawLRempty}{\coordinate (LR) at ( \boxsize, -\boxsize);}
\newcommand{\drawLLempty}{\coordinate (LL) at (-\boxsize, -\boxsize);}

\newcommand{\drawboxinternallines}{
  \draw (UL) -- (UR) -- (LR) -- (LL) -- (UL);
}

\newcommand{\drawinternalmomenta}{
  \draw[->] (+0.3, -1.1) -- (-0.3, -1.1) node[anchor=north west] {$\lone$};
  \draw[->] (-1.1, -0.3) -- (-1.1, +0.3) node[anchor=north east] {$\ltwo$};
  \draw[->] (-0.3, +1.1) -- (+0.3, +1.1) node[anchor=south east] {$\lthree$};
  \draw[->] (+1.1, +0.3) -- (+1.1, -0.3) node[anchor=south west] {$\lfour$};
}

\newcommand{\drawregionvariables}[5]{
  \draw ( 0.0, -1.4) node {#1};
  \draw (-1.4,  0.0) node {#2};
  \draw ( 0.0,  1.4) node {#3};
  \draw ( 1.4,  0.0) node {#4};
  \draw ( 0.0,  0.0) node {#5};
}

%%%%% BCFW %%%%%%

\newcommand{\drawLblack}{\node[circle, fill=black, draw, minimum size=0.3cm] (L) at (-0.9,  0.0) {};}
\newcommand{\drawRblack}{\node[circle, fill=black, draw, minimum size=0.3cm] (R) at ( 0.9,  0.0) {};}

\newcommand{\drawLwhite}{\node[circle, fill=white, draw, minimum size=0.3cm] (L) at (-0.9,  0.0) {};}
\newcommand{\drawRwhite}{\node[circle, fill=white, draw, minimum size=0.3cm] (R) at ( 0.9,  0.0) {};}

\newcommand{\drawL}[1]{\node[circle, fill=black!20, draw, minimum size=0.5cm, inner sep=2pt] (L) at (-0.9,  0.0) {#1};}
\newcommand{\drawR}[1]{\node[circle, fill=black!20, draw, minimum size=0.5cm, inner sep=2pt] (R) at ( 0.9,  0.0) {#1};}

\newcommand{\drawBCFWinternalline}{
  \draw (L) -- ++( 0.8,  0.0);
  \draw (R) -- ++(-0.8,  0.0);
}

%%%%% MHV %%%%%%

\newcommand{\drawblobs}{
\node[circle, fill=black!20, draw, minimum size=0.6cm] (blobL) at (-1, 0) {};
\node[circle, fill=black!20, draw, minimum size=0.6cm] (blobR) at (+1, 0) {};
}

\newcommand{\drawupperlower}{
\draw (blobL) to[out=60, in=120] (blobR);
\draw (blobL) to[out=-60, in=-120] (blobR);
}

\newcommand{\drawuppercross}{
\draw (blobL) to[out=60, in=120] node[cross out, draw=red]{} (blobR);
}

\newcommand{\drawlowercross}{
\draw (blobL) to[out=-60, in=-120] node[cross out, draw=red]{} (blobR);
}

\newcommand{\drawuppercut}{
\draw (blobL) to[out=60, in=120] node[circle, fill=white, draw=white]{} (blobR);
\draw[red, dashed] (0, 0.4) -- (0, 1.0);
}

\newcommand{\drawlowercut}{
\draw (blobL) to[out=-60, in=-120] node[circle, fill=white, draw=white]{} (blobR);
\draw[red, dashed] (0,-0.4) -- (0,-1.0);
}

